An Offline Meta Black-box Optimization Framework for Adaptive Design of Urban Traffic Light Management Systems

Complex urban road networks with high vehicle occupancy frequently face severe traffic congestion. Designing an effective strategy for managing multiple traffic lights plays a crucial role in managing congestion. However, most current traffic light management systems rely on human-crafted decisions, which may not adapt well to diverse traffic patterns. In this paper, we delve into two pivotal design components of the traffic light management system that can be dynamically adjusted to various traffic conditions: phase combination and phase time allocation. While numerous studies have sought an efficient strategy for managing traffic lights, most of these approaches consider a fixed traffic pattern and are limited to relatively small road networks. To overcome these limitations, we introduce a novel and practical framework to formulate the optimization of such design components using an offline meta black-box optimization. We then present a simple yet effective method to efficiently find a solution for the aforementioned problem. In our framework, we first collect an offline meta dataset consisting of pairs of design choices and corresponding congestion measures from various traffic patterns. After collecting the dataset, we employ the Attentive Neural Process (ANP) to predict the impact of the proposed design on congestion across various traffic patterns with well-calibrated uncertainty. Finally, Bayesian optimization, with ANP as a surrogate model, is utilized to find an optimal design for unseen traffic patterns through limited online simulations. Our experiment results show that our method outperforms state-of-the-art baselines on complex road networks in terms of the number of waiting vehicles. Surprisingly, the deployment of our method into a real-world traffic system was able to improve traffic throughput by 4.80\% compared to the original strategy.

==> algorithms/bo.tex <==
\begin{figure}[h]
\centering
\begin{minipage}[t!]{0.9\linewidth}
\centering
\begin{algorithm}[H]
\small
\begin{spacing}{1.0}
\caption{Bayesian Optimization}
\label{alg:bo}
\small
\begin{algorithmic}
\State 
Given black-box function $f$ and online evaluation budget $T$
\State
Initialize surrogate model $S_{0}$ and acquisition function $A$
\State
Set $\mathcal{D} \gets \emptyset$
\For{$t=1,\ldots, T$} 
    \State Choose $\mathbf{x}_{t} \gets \arg\min_{\mathbf{x}} A(\mathbf{x}, S_{t-1})$
    \State Evaluate $\mathbf{x}_{t}$ and get $f(\mathbf{x}_{t})$
    \State Update $\mathcal{D} \gets \mathcal{D} \cup \{(\mathbf{x}_t, y_{t})\}$
    \State Update surrogate model $S_{t} \gets S_{t-1}$ using $\mathcal{D}$
\EndFor
\State Choose the best $\mathbf{x}^{*}$ in $\mathcal{D}$
\end{algorithmic}
\end{spacing}
\end{algorithm}
\end{minipage}
\end{figure}

==> tables/ablation3.tex <==
\begin{table}[t]
\centering
\caption{Experiment Results on Extreme Traffic Scenarios. Experiment is conducted on phase time allocation task}
% \vspace{-7pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Average Number of Waiting Vehicles ($\downarrow$)}}\\ 
\cmidrule{2-5}
& Grid\_2$\times$2 & Grid\_3$\times$3 & Grid\_4$\times$4 & Grid\_5$\times$5 \\
\midrule
% timing
RGPE & 60.78 ± 2.82& 167.92 ± 0.84& 297.30 ± 2.18&468.78 ± 2.79\\
ABLR & 55.48 ± 1.57& 160.74 ± 1.81& 285.17 ± 1.64&459.05 ± 8.41\\
FSBO & 54.51 ± 0.82& 162.56 ± 0.66& 287.26 ± 0.82&467.42 ± 2.45\\
\bottomrule
Ours & 53.44 ± 1.31& 164.67 ± 0.46& 284.25 ± 3.03&465.91 ± 3.64\\
\bottomrule
\end{tabular}
}
\label{table:ablation3}
\end{table}

==> tables/data_collection.tex <==
\begin{table}[t]
\centering
\caption{Comparison of different data collection strategies.}
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Average Number of Passing Vehicles ($\uparrow$)}}\\
\cmidrule{2-5}
  & Tue & Wed & Thu & \textbf{Overall}\\
\midrule
Fixed Time (veh/hr) & 16775 & 16072 & 19185 &\textbf{17344}\\
Ours (veh/hr)   & 17672 & 17735 & 19120 &\textbf{18176}\\
\midrule
Improvement (\%)	&	5.35	& 10.35 & -0.34 &\textbf{4.80}\\
\bottomrule
\end{tabular}
\label{table:data_collection}
\end{table}

==> tables/districtA_info.tex <==
\begin{table}[h]
\centering
\caption{Details on optimized traffic signals in District A}
\vspace{-7pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc}
\toprule
 \textbf{Intersection ID} & \# of Phases & Min Green Time & Cycle Time\\
\midrule
1	&	3	& 75/36/34 & 160\\
2	&	4	& 79/18/30/18	&	160\\
3	&	4	& 74/18/34/18	&	160\\
4	&	4	& 64/17/31/31	&	160\\
5	&	4	& 84/17/13/30 & 160\\
6	&	4	& 61/17/38/29 & 160\\
7	&	4	& 71/18/28/28 & 160\\
8	&	4	& 71/18/28/28 & 160\\
9	&	4	& 27/70/16/32 & 160\\
10	&	5	& 22/47/34/24/17 & 160\\
11	&	3	& 69/10/38 & 130\\
12	&	3	& 63/21/33 & 130\\
13	&	3	& 60/35/22 & 130\\
14	&	4	& 48/44/44/31 & 185\\
15	&	3	& 126/22/18 & 185\\
16	&	3	& 48/24/27 & 110\\
17	&	5	& 57/49/18/25/13 & 180\\
18	&	4	& 80/40/28/13 & 180\\
19	&	3	& 115/18/29 & 180\\
20	&	5	& 27/36/41/21/36 & 180\\
21	&	5	& 45/45/21/26/26 & 180\\
22	&	5	& 45/40/21/27/29 & 180\\
23	&	5	& 54/38/16/27/26 & 180\\
24	&	5	& 33/35/36/30/29 & 180\\
25	&	5	& 48/37/12/35/30 & 180\\
26	&	3	& 74/27/62 & 180\\
\bottomrule
\end{tabular}}
\label{table:districtA_info}
\end{table}

==> tables/offset.tex <==
\begin{table*}[t]
\centering
\caption{Performance of all methods on optimizing offset}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{clcccc|ccc}
\toprule
\multirow{3}{*}{\textbf{Framework}} & \multirow{3}{*}{\textbf{Method}} & \multicolumn{7}{c}{\textbf{Average Number of Waiting Vehicles ($\downarrow$)}}\\ 
\cmidrule{3-9}
% & & \multicolumn{5}{c|}{Synthetic Dataset} & \multicolumn{2}{c}{Public Real-world Dataset}\\
% \cmidrule{3-9}
& & Grid\_2$\times$2 & Grid\_3$\times$3 & Grid\_4$\times$4 & Grid\_5$\times$5 & Hangzhou\_4$\times$4 & Manhattan\_16$\times$3 & Manhattan\_28$\times$7\\
\midrule
\multirow{6}{*}{Online BBO} 
& GA & & & & & & & \\
& PSO & & & & & & & \\
& CMA-ES & & & & & & & \\
& GP-UCB & & & & & & & \\
& REINFORCE & & & & & & & \\
& PPO & & & & & & & \\
\midrule
\multirow{3}{*}{Offline BBO} 
& CbAS & & & & & & & \\
& COMs & & & & & & & \\
& MINs & & & & & & & \\
\midrule
\multirow{4}{*}{Meta BBO} 
& LGA & & & & & & & \\
& LES & & & & & & & \\
& RGPE & & & & & & & \\
& FSBO & & & & & & & \\
\midrule
\multirow{1}{*}{Offline Meta BBO} 
& Ours & & & & & & & \\
\bottomrule
\end{tabular}}
\label{table:exp_offset}
\end{table*}
